Persona-L has Entered the Chat: Leveraging LLM and Ability-based Framework for Personas of People with Complex Needs

We present Persona-L, a novel approach for creating personas using Large Language Models (LLMs) and an ability-based framework, specifically designed to improve the representation of users with complex needs. Traditional methods of persona creation often fall short of accurately depicting the dynamic and diverse nature of complex needs, resulting in oversimplified or stereotypical profiles. Persona-L enables users to create and interact with personas through a chat interface. Persona-L was evaluated through interviews with UX designers (N=6), where we examined its effectiveness in reflecting the complexities of lived experiences of people with complex needs. We report our findings that indicate the potential of Persona-L to increase empathy and understanding of complex needs while also revealing the need for transparency of data used in persona creation, the role of the language and tone, and the need to provide a more balanced presentation of abilities with constraints.

==> Sections/FigureDescription.tex <==
Figure 1: “Persona-L interface. This figure shows the Persona-L interface, featuring a chat window where users can interact with Persona-L through conversation.”
Figure 2: “System Design Diagram. This diagram maps the journey from data collection to Persona-L creation, highlighting the key processes involved. The dataset is processed through data collection, theme categorization, and ground truth question formulation. This dataset is then used for LLM model training and Persona-L interface development, which includes profile generation, ability exploration, and persona interaction. Finally, the user interface and LLM model are integrated through back-end APIs, persona creation API and persona chat API."
Figure 3: "Phases in User Interface Design: This figure displays three key phases of the Persona-L system. The "Profile Phase" involves persona customization and theme selection. The "Ability Phase" allows users to explore and select key abilities under specific theme. The "Interaction Phase" facilitates user engagement with the personas LLMs and provides tools for saving and documenting interactions."
Figure 4: "This figure shows the Profile Phase Page. The left side of the page contains fields and drop-downs for selecting attributes such as age, gender, occupation, medical condition, and themes (e.g., employment, education) to create a persona. The right side displays the persona profile, including an image, name, age, gender, occupation, medical condition, theme, and a brief description."
Figure 5: "This figure displays a page in Persona-L where users can view the key abilities associated with a persona under the Employment theme. The screen shows a list of abilities, with details such as the ability name, description, ability drivers (e.g., tools or environments that enhance the ability), and ability blockers (e.g., challenges the persona faces)."
Figure 6: "This figure depicts the Interaction Phase, where users can chat with the persona. The conversation window is prominently displayed, showing the persona's responses to user questions. When users summarize their conversations, a summary page is loaded. Users can scroll through chat history, save the interview, add design goals to the background section, or restart the interview. The features on the Interaction Phase page includes: (1) Pre-defined questions (2) Chat with Persona-L (3) Mark questions (4) Historical chats (5) Summarize questions (6) Detailed Interview scripts (7) Persona Library"

Table 1: "Example of an Ability Name, Ability Driver, and Ability Blocker for the Employment Theme.
This table provides an example from the Employment theme, detailing one persona's ability (e.g., Memory Skills), along with descriptions of ability drivers (e.g., visual and auditory aids) and ability blockers (e.g., complex information). It includes a brief story illustrating how each driver and blocker affects the persona’s ability to perform tasks."
Table 2: "Participant Demographics and Experience Summary. This table lists the demographics and professional experience of participants in the user study, including their id, age, gender, country, occupation, and years of experience."
Table 3: "Interaction Scenarios for user study. This table outlines specific scenarios under the themes of employment, education, and family, detailing the situations, interactions, and goals of engaging with personas representing individuals with Down syndrome."
Table 4: "Interview questions. This table contains a list of interview questions used during the user study. The questions focus on participants' experience with persona creation, their familiarity with people with Down syndrome, and their interactions with Persona-L."
Table 5: "Example of One Data Entry Extracted from Real People’s Stories. This table shows an example of a data entry extracted from real stories of people with Down syndrome. The entry includes name, diagnosis, resources, age, gender, region, education, occupation, family situation, label, abilities, and challenges."
Table 6: "Persona Creation API. This table shows the persona creation API example including request body, request example, response body, and response example in JSON format."
Table 7: "Persona Chat API. This table shows the persona chat API example including request body, request example, response body, and response example in JSON format."
Table 8: "Example Prompts for LLM Persona Generation Strategies. This table presents four prompting strategies: general guidelines, role-play prompting, on-shot prompting, and incremental prompting, each with an example."
Table 9: "User story for interaction phase. This table outlines a user story for the Interaction Phase, including features, needs, and purposes. Features include pre-defined questions, chat with LLMs, mark questions, historical chats, summarize questions, persona library, and detailed interview scripts."

==> Sections/User_Study_1.tex <==
\section{User Study 1: Comparison of static vs interactive LLM personas}



REMOVE EVERYTHING EXCEPT QUAL<
REVISE QUESTIONS AND ASK DESIGNERS

We conducted an exploratory user study designed to evaluate the quality of the personas created with our system. We also compared compare the interactive personas generated by our interface with traditional static personas in the user study. The user study process is shown in Figure 6. \\

\subsection{Participants}
We recruited 10 participants with UX, product design and software design backgrounds and prior experience with personas and large language models such as ChatGPT and Bard. Their familiarity with these concepts is essential for providing informed and relevant feedback to our system. Each participant was thoroughly briefed about the objectives of the study. %This recruitment strategy would help ensure that our study benefits from a range of perspectives, enhancing the reliability and applicability of our findings.

\subsection{Procedures}
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{6-2.png}
    \caption{Procedure of User Study. After the 1. Pre-study preparation, target users 2. select and explore a static persona and 3. interact with the personas generated by our interface. 4. Then post-trial surveys and semi-structure interviews will be conducted. quantitative and qualitative data will be collected and analyzed.}
    \label{fig:enter-label}
\end{figure}
\subsubsection{Pre-study Preparation:} Initially, we developed a series of scenarios (see Table \ref{tab:scenarios}) as design briefs. These scenarios are categorized into three themes: employment, education, and family, each tailored to our interface's structure and knowledge base previously gathered. Table \ref{tab:scenarios} provides detailed descriptions, including specific situations, interactions, and objectives for each scenario. We have used ChatGPT-4o to generate a persona profile for each scenario (see Appendix \ref{PersonaProfiles}), allowing users to select one Persona Profile along with its corresponding scenario. 

\subsubsection{Study Task: Evaluating Personas} Participants were tasked with selecting one of the previously prepared scenarios (see Table \ref{tab:scenarios}) and one of the Persona Profiles (see Appendix \ref{PersonaProfiles}). After they made a selection they were given 8 minutes to come up with design ideas specific to the chosen scenario. After this exercise, participants were asked to select another scenario and this time were given our Persona interface. Participants were instructed to explore its various functionalities present in all three phases: Profile, Ability, and Interaction (see Figure \ref{fig:Phases}), and build a persona that matches criteria in a chosen scenario. After Persona was created participants were given 8 minutes to ideate new designs for the chosen scenario. The rationale for approach is in our intention to facilitate a comparative analysis between the predefined Persona Profiles and personas generated by our system, assessing whether the interactive Personas offers enhanced contextual understanding and added value to the design process.

\begin{table}
    \centering
    \begin{tabular}{|c|p{0.2\textwidth}|p{0.4\textwidth}|p{0.3\textwidth}|}\hline
         Theme&  Situation&  Design Task& Design Goal\\ \hline 
         Employment&  Seeking for a Job &  You want to know what can help people with Down syndrome when they are looking  to find a job.
Engage with the given persona to understand their experience when finding a job, help received from individuals and social groups, and suggestions from their lived experiences.& The goal is to gain insights into communication strategies and support systems that can aid individuals with Down syndrome in job seeking and workplace integration.\\ \hline 
         Employment&  Career Development &  You are interested in learning about career advancement opportunities for individuals with Down syndrome. 
Engage with the given persona to learn their personal experiences with various training programs, mentoring relationships, and career advancement strategies that have supported their professional growth.& The goal is to propose better services that  can facilitate effective communication and mentorship opportunities and support career development and long-term engagement for employees with Down syndrome.\\ \hline 
         Employment&  Enhancing Work Efficiency &  You want to explore how work efficiency can be enhanced specifically for individuals with Down syndrome. 
Engage with the given persona to learn the types of tools, technologies, and products that have significantly improved their productivity and job performance.& The goal is to gather information about new communication features or products that could be developed or adapted to help individuals with Down syndrome work more effectively and independently.\\ \hline 
         Education&  Learning at School&  You aim to understand the specifics of learning experiences at school for individuals with Down syndrome. 
Engage with the given persona to understand the methods of learning, challenges faced, and strategies to overcome these challenges.& The goal is to design educational tools or curricula that are better suited to enhance communication and learning experiences for individuals with Down syndrome.\\ \hline 
         Family&  Interacting with Family&  You seek to understand the day-to-day interactions within the family setting for individuals with Down syndrome, especially how they communicate with their family members. 
Engage with the given persona to learn methods of communication, and how they establish and maintain family relationships.& The goal is to design more inclusive and supportive family communication tools or strategies.\\ \hline
    \end{tabular}
    \caption{Interaction Scenarios for user study. This table outlines specific scenarios under the themes of employment, education, and family, detailing the situations, interactions, and goals of engaging with personas representing individuals with Down Syndrome.}
    \label{tab:scenarios}
\end{table}


\subsection{Data Collection} 
After the above procedures, participants participated in a brief semi-structured interview. We focused our open-ended questions in the interview to specifically focus on comparing predefined Persona Profiles and the interactive personas generated by our interface. These question aim to explore how interactions with our personas influence the design process, the understanding of specific user groups such as individuals with Down syndrome, the unique insights provided by interactive personas, the practical features of our interface, and overall satisfaction with the interface.(open-ended questions details provided in Table \ref{tab:openEndedQuest}). 
\begin{table}
    \centering
    \begin{tabular}{|c|p{0.85\textwidth}|} \hline  
         Q1& Compared to static personas, what are the advantages and disadvantages of interactive personas generated by our interface? Please provide an example from your interaction to illustrate your point of view.\\ \hline  
         Q2& Can you describe how interacting with the persona has influenced your design process for these personas? Please provide an example of a design decision that was directly influenced by feedback from an interactive persona?\\ \hline 
          Q3& Compared to static personas, do you think the interaction process with interactive personas allows you to better understand individuals with Down syndrome? Why? Please provide examples to illustrate this.\\ \hline 
         Q4& Can you describe a scenario where an interactive persona provided insights that you believe a static persona would not have revealed?\\\hline   
         Q5& Compared to traditional methods of persona creation, what features of our interface do you find most practical? Can you provide an example that illustrates the utility of these features in enhancing your interaction with the personas?\\ \hline  
         Q6& Reflecting on your entire experience, how satisfied are you with the interface? What features added or changes made would increase your satisfaction? \\ \hline
    \end{tabular}
    \caption{Open-ended questions}
    \label{tab:openEndedQuest}
\end{table}

By allowing users to freely share their thoughts, we gain deeper insights into the subjective experiences and potential improvements, enriching the feedback loop necessary for refining our system. This approach not only helps validate our quantitative findings but also uncovers rich, qualitative data that can guide further development and enhancements of our interface and personas.

\subsection{Data Analysis}  
To analyze the qualitative data collected from open-ended questions, we conducted a thematic analysis \cite{braun2012thematic}. We designed open-ended questions to compare interactive personas generated by our interface and static personas. We initially identified codes within the responses, which were then grouped into broad themes. Appendix B Table 10 presents the thematic categorizations corresponding to various questions, outlining the codes utilized to categorize the responses.
%\subsection{Data Analysis}
%The data analysis for this study have been conducted in several stages to ensure a comprehensive understanding of both the quantitative and qualitative feedback collected from the participants. 
  %  \begin{itemize}
     %   \item \textbf{Descriptive Statistics:} We calculated means, standard deviations, and frequency distributions for the quantitative survey responses to get a preliminary understanding of the data, highlighting immediate trends or anomalies.
    %    \item \textbf{Key Metrics Analysis: }We compiled and analyzed the ratings for each key metric, summarizing the results to identify trends, averages, and variances. This analysis enabled us to pinpoint the strengths and weaknesses of various contextual aspects of the interface and personas, informed by user feedback. 
      %  \item \textbf{Integration with Quantitative Findings:} The quantitative data evaluation of key metrics has been combined with qualitative insights to mutually validate the findings and provide a more comprehensive understanding of user feedback.
    % \item \textbf{Qualitative Data Analysis: }
    % \begin{itemize}
    %     \item \textbf{Focused Metric Analysis}: For each specific question, responses will be extracted and common experiences and problems expressed by participants will be highlighted. This targeted analysis aids in understanding the specific aspects of the interface or persona that resonate most with users, facilitating a deeper comprehension of their needs and expectations.
    %     \item \textbf{Integration with Quantitative Findings:} The themes identified will be compared with quantitative data to explore correlations and variances between subjective perceptions and objective scores. This helps in validating the qualitative findings with quantitative measures.
    % \end{itemize}
    %\end{itemize}



\section{Findings} 
%\subsection{Metrics Analysis} 
  %  \begin{figure}
  %      \centering
   %     \includegraphics[width=1\linewidth]{metrics_interface.png}
  %      \caption{Average scores for metrics that assess the richness of context for the interface, with error bars indicating the standard error}
 %  \end{figure}  
  %      \begin{figure}
   %     \centering
   %     \includegraphics[width=1\linewidth]{metrics_persona.png}
   %     \caption{Average scores for metrics that assess the richness of context for the persona, with error bars indicating the standard error}
  %  \end{figure} 
  %  We consolidate various questions into distinct metrics to calculate average scores and standard errors. As illustrated in Figure 7 and Figure 8, except Contextual Adaptability in Persona, other metrics scores are all above 4.0, indicating that participants generally agree or rate positively on the statements. The uniformity of the small error bars across all metrics suggests consistent participant responses with minimal outliers. For the interface, \textbf{User Satisfaction} is notably high (mean=4.53, std=0.63), and \textbf{User Satisfaction} for Persona (mean=4.1, std=0.57), which suggests participants are generally satisfied with our system and likely to recommend it. For specific metrics, Interface has the highest scores in \textbf{Contextual Completeness} (mean=4.5, std=0.57) and \textbf{Contextual Adaptability} (mean=4.5, std=0.57), indicating the interface provides a comprehensive context that can be adapted to meet various participant requirements. However, In the persona category, the highest score is observed in \textbf{Contextual Consistency} (mean=4.4, std=0.52), and the lowest score is in \textbf{Contextual Adaptability} (mean=3.8, std=0.92), the second lowest score is in \textbf{Contextual Accuracy} (mean=4.0, std=0.56), which indicates that the responses of LLMs are consistent with the description of personas but the adaptability of these responses to various themes and abilities as well as the accuracy needs to be improved. 
%\subsection{Granular Analysis of Metric Questions}   
  %  \begin{figure}
   %     \centering
   %     \includegraphics[width=1\linewidth]{questions_interface.png}
   %     \caption{Average scores for specific questions comprising metrics in the interface category, accompanied by error bars representing the standard error}
  %  \end{figure}   
     %   \begin{figure}
    %    \centering
    %%    \includegraphics[width=1\linewidth]{questions_persona.png}
    %    \caption{Average scores for specific questions comprising metrics in the persona category, accompanied by error bars representing the standard error}
  %  \end{figure}  
   % Figure 9 and 10 present bar charts illustrating average scores for various questions associated with the Interface and Persona categories. These questions, possibly singular or multiple, comprise various metrics. Scores predominantly hover around 4.0 or higher, and the minimal error bars indicate a uniform agreement among participants on each statement. The uniformly high scores of Interface-related questions indicate that participants were generally satisfied with the contextual aspects of the interface. In addition, Q1 (mean=4.5, std=0.53) and Q5 (mean=4.5, std=0.53) have the same high scores, and they both represent statements about the adequacy of ability's descriptions, drivers, and blockers providing a rich context, indicating that participants are receptive to the ability-based framework. For Persona, Q4 (mean=3.9, std=0.32) and Q5 (mean=3.8, std=0.92) record scores lower than 4.0, Q4 pertains to the statement that the persona provides sufficiently accurate and reliable information, while Q5 relates to the persona's adaptability to changes in themes and abilities. This implies that participants may have reservations about trusting the persona and its responses, given concerns about its adaptability and accuracy. 



Analysis of collected interview data yielded following key themes :  \textbf{Increased Empathy}, \textbf{Adaptability}, \textbf{Completeness of Information}, and \textbf{Real-Time Interaction} to demonstrate the advantages of our interactive persona compared to the static persona. Participants also offered some advice such as \textbf{More Guidance}, \textbf{Low Relevance}, and \textbf{Misrepresentation}, which become learning inputs indicating our future work.    
\subsubsection{Increased Empathy} 
Participants felt the interaction allowed for a more detailed and empathetic understanding of individuals with Down syndrome, especially combined with demonstrated abilities.\textit{"The emotional response and specific situation wouldn't have been captured in a static persona, which reflects individual variability and real-time emotional states."} (P4). P2 also mentioned that using a static persona is like reading articles, which is boring and hard to go through the information she needs.
\subsubsection{Adaptability}  
Participants agreed that one of the most practical features of the interface is the ability to dynamically update and adapt personas based on interactions. \textit{"This allows for a more personalized and accurate representation of user needs, users can adjust questions in real-time to dive deeper into the target persona's experience"} (P4). P3 thought the ability to simulate scenarios was impressive, \textit{"For example, by simulating a job-seeking scenario, I can interact with a shopping assistant and adjust the support features accordingly"}. Moreover, pre-defined questions allow users to adapt the conversation based on the persona’s background and current theme, enabling users to explore various aspects of a persona's professional and personal life more effectively, \textit{"The feature that stands out is the provision of pre-set example questions during interactions with the personas. For instance, when interacting with a persona who works in retail, the example questions helped me delve into specific scenarios like handling customer complaints or managing stress during peak hours. This not only made the interaction more structured but also allowed me to gather insights that would be crucial for designing a more accessible and user-friendly environment for individuals with similar profiles"} (P7).
\subsubsection{Completeness of Information}  
Almost all participants mentioned that the interactive persona provides more detailed information, which expands the brief description of static personas. \textit{"Interacting with the persona can help me understand the life details of the group it represents. For example, when I was designing products for individuals with Down syndrome in a workplace environment, the persona told me that they prefer products with visual designs to improve work efficiency. This gives me inspiration for my product design}" (P8). The ability model is a vital feature that enhances the understanding of the persona, \textit{"The introduction of ability shows me what individuals with Down syndrome enjoy. It was unclear to me before"} (P5), \textit{"The most practical feature is the ability driver. It tells me what the personas have advantages in"} (P6).
\subsubsection{Real-Time Interaction}  
Participants emphasized that interactive personas have deeply influenced the design process by providing real-time feedback to directly address specific needs. P3 illustrated an example, \textit{"I want to design a persona for a shop assistant with Down syndrome. In an interactive persona, he expresses confusion and provides real-time feedback on what help he needs and what remains confusing, whereas a static persona can provide"}. P7 had a scenario in which a persona worked in a retail store and encountered communication difficulties. In this situation, a static persona can only provide general information about their communication styles, however, an interactive one could respond directly to queries about what would help them most during such a stressful interaction. The real-time adaptability and specificity make interactive personas particularly valuable in designing supportive environments tailored to individual needs.
\subsubsection{More Guidance}  
Participants expressed a desire for more guided interactions within the persona system. \textit{"Adding features like providing more example questions that can differentiate individuals with Down syndrome and others will help increase my satisfaction"} (P5), \textit{"I think it would be even better if the interface could provide some guidance on product design questions"} (P8). Providing additional sample questions specifically tailored to product design can offer clearer pathways for exploration, and further guidance should be offered to enhance understanding of Down Syndrome. 
\subsubsection{Low Relevance} 
There are also concerns about the relevance and accuracy of the personas, P7 found the persona lacked cohesion, \textit{"An interesting aspect of the interactive persona is sharing specific future career aspirations like owning a tattoo shop, which contrasts with her current job as a cook"}, P10 observed significant homogeneity in the personas, \textit{"When I create multiple personas and ask them the same question—how their interests affect their career—they exhibit a high degree of similarity in their interests"}.  
\subsubsection{Misrepresentation}  
Some participants raised issues regarding the authenticity of the current personas. P3 and P10 felt that some of the responses lacked realism, while P3 and P4 described them as too generic. P1 commented that the interactive persona system showed limited improvement because it was overly positive, failing to capture the complexities of real-life situations. P6 said: \textit{"I was surprised that the patient said his disease enhanced his creativity, which seems quite weird"}. This overly optimistic portrayal led to personas that seemed unrealistic and disconnected from the true experiences of individuals. 
